Stochastic Multiple Target Sampling Gradient Descent

Sampling from an unnormalized target distribution is an essential problem with many applications in probabilistic inference. Stein Variational Gradient Descent (SVGD) has been shown to be a powerful method that iteratively updates a set of particles to approximate the distribution of interest. Furthermore, when analysing its asymptotic properties, SVGD reduces exactly to a single-objective optimization problem and can be viewed as a probabilistic version of this single-objective optimization problem. A natural question then arises: "Can we derive a probabilistic version of the multi-objective optimization?". To answer this question, we propose Stochastic Multiple Target Sampling Gradient Descent (MT-SGD), enabling us to sample from multiple unnormalized target distributions. Specifically, our MT-SGD conducts a flow of intermediate distributions gradually orienting to multiple target distributions, which allows the sampled particles to move to the joint high-likelihood region of the target distributions. Interestingly, the asymptotic analysis shows that our approach reduces exactly to the multiple-gradient descent algorithm for multi-objective optimization, as expected. Finally, we conduct comprehensive experiments to demonstrate the merit of our approach to multi-task learning.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}

==> related_work.tex <==
 The work of \cite{desideri2012multiple} proposed a multi-gradient
descent algorithm for multi-objective optimization (MOO) which opens
the door for the applications of MOO in machine learning and deep
learning. Inspired by \cite{desideri2012multiple}, MOO has been applied
in multi-task learning (MTL) \cite{sener2018multi,mahapatra2020multi},
few-shot learning \cite{ye2021multi}, and knowledge distillation
\cite{du2020agree}. Specifically, the work of \cite{sener2018multi}
viewed a multi-task learning as a multi-objective optimization problem,
where a task network consists of a shared feature extractor and a
task-specific predictor. The work of \cite{mahapatra2020multi} developed
a gradient-based multi-objective MTL algorithm to find a solution
that satisfies the user preferences. The work of \cite{lin2019pareto}
proposed a Pareto MTL to find a set of well-distributed Pareto solutions
which can represent different trade-offs among different tasks. Recently,
the work of \cite{liu2021profiling} leveraged MOO with Stein Variational
Gradient Descent \cite{liu2016stein} and Langevin dynamics \cite{welling2011bayesian} to diversify the solutions of
MOO. Additionally, the work of \cite{ye2021multi} proposed a bi-level
MOO which can be applied to few-shot learning. Finally, the work of
\cite{du2020agree} applied MOO to enable the knowledge distillation
from multiple teachers.

